MeshFleet: Filtered and Annotated 3D Vehicle Dataset for Domain Specific Generative Modeling

Generative models have recently made remarkable progress in the field of 3D objects. However, their practical application in fields like engineering remains limited since they fail to deliver the accuracy, quality, and controllability needed for domain-specific tasks. Fine-tuning large generative models is a promising perspective for making these models available in these fields. Creating high-quality, domain-specific 3D datasets is crucial for fine-tuning large generative models, yet the data filtering and annotation process remains a significant bottleneck. We present MeshFleet, a filtered and annotated 3D vehicle dataset extracted from Objaverse-XL, the most extensive publicly available collection of 3D objects. Our approach proposes a pipeline for automated data filtering based on a quality classifier. This classifier is trained on a manually labeled subset of Objaverse, incorporating DINOv2 and SigLIP embeddings, refined through caption-based analysis and uncertainty estimation. We demonstrate the efficacy of our filtering method through a comparative analysis against caption and image aesthetic score-based techniques and fine-tuning experiments with SV3D, highlighting the importance of targeted data selection for domain-specific 3D generative modeling.

==> archiv/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}

Recent advances in 3D generative modeling have shown remarkable potential for creating realistic and diverse 3D content from text or reference images\cite{xiang2024structured, voleti2024sv3d, xu2024instantmesh, liu2023zero1to3, shi2023zero123plus, hunyuan3d22025tencent, yang2024hunyuan3d}. However, the performance of these models is highly dependent on the quality and relevance of the training data. Although large-scale 3D datasets like Objaverse-XL \cite{objaverseXL} offer unprecedented data volume, they also contain a significant proportion of noisy or irrelevant samples, necessitating careful filtering and annotation \cite{voleti2024sv3d, xiang2024structured}. 

This problem is exaggerated in industrial applications for engineering and creative design applications. These areas require high levels of detail, symmetry, and object consistency within specific domains. Adherence to specific design constraints and controlability is crucial. An example of this is a 3D generative model for the vehicle design process. During vehicle design, many factors influence decision making, from technical aspects to aesthetics. Many steps and evaluations are based on models with different amounts of detail. 

For example, the shape of the vehicle is fundamental for the final design and perceived aesthetics, while also having an important impact on the efficiency of the resulting vehicle. Both are factors car manufacturers wish to optimize. Simulative drag testing in the early stages can reduce the number of design iterations, while also improving the final result of the design process. The simulation of drag often relies on the shape of the vehicle, where the accuracy of the estimate increases with the accuracy of the shape. Generating shapes based on general inputs can reduce the amount of manual labor in early stages and, therefore, improve the efficiency of the design process. Ideally such a generative model would be able to create 3D shapes of vehicles without any artefacts while adhering to the description and technical conditioning as well as generating high fidelity and visually appealing objects. Additionally high fidelity 3D models can also improve the communication and visualization of design concepts. While high fidelity domain specific 3D generative models are ambitios, moving towards such generative models could revolutionise the whole design process in many areas. 

%---- Gap of existing approaches
However, the availability of datasets in these specialized domains is often limited, with realistic sizes ranging from a few hundred to a few thousand objects. The general amount of vehicles and vehicle-like objects in Objaverse and Objaverse-XL \cite{objaverse, objaverseXL} is high, with an estimate of more than 20,000 captions from Cap3D \cite{luo2024view, luo2023scalable} and TRELLIS500K\cite{xiang2024structured} depicting cars. However, the actual number of high-quality vehicles which satisfy the requirements for fine-tuning a model for design applications is much lower, the exact number of these objects being unclear. The manual curation of such datasets is time-consuming and expensive, hindering rapid progress in the field of 3D generative models for specific domains or with special conditioning.

To address these challenges, we propose MeshFleet, an annotated 3D vehicle dataset derived from Objaverse-XL. The dataset consists of two parts. The first part is the manually labeled subset of Objaverse \cite{objaverse} which was collected by automatically detecting vehicles using images of objects. Each object was then hand-labeled with how well it is suited to fine-tune a model on generating high quality vehicles. The second part of the dataset was generated using an automated pipeline that processed and classified objects from Objaverse-XL. Resulting in more than one million ($1059727$) processed objects from the Objaverse Alignment dataset \cite{objaverseXL} and TRELLIS500K\cite{xiang2024structured}. Based on these, we collected $1620$ high-quality vehicles. We define a high-quality vehicle as a single 3D object that is a well-defined car with recognizable make and model, exhibiting detailed contours and representative features.

We trained an initial quality classifier based on DINOv2\cite{oquab2024dinov2} features and SigLIP \cite{zhai2023siglip} embeddings using the manually labeled subset. This classifier automatically identifies and filters out low-quality or non-vehicle objects from Objaverse-XL. We then refine the filtering results by analyzing the object descriptions of CAP3D\cite{luo2023scalable} and TRELLIS500K\cite{xiang2024structured}, identifying and correcting misclassifications. We also incorporate uncertainty estimation techniques to collect further data in order to improve the robustness of the classifier. Our final model classifies high-quality vehicles with an accuracy of $95\%$ using $6200$ labeled objects. The finally filtered $1620$ vehicles were manually assessed to ensure that all objects are indeed high quality cars. The filtered objects were further processed to generate captions and size estimates for all vehicles. 

We validate the effectiveness of our labeling and filtering method by fine-tuning SV3D \cite{voleti2024sv3d}, a state-of-the-art multiview generative model, on the filtered datasets and comparing the results with those obtained using other filtering strategies. The results demonstrate that finetuning on high-quality objects results in increased quality and multi-view-consistency of the domain-specific generated objects. This underlines that data quality is preferable over data quantity. Finetuning SV3D on significantly fewer, high-quality objects yields better model performance than finetuning on more objects with lower quality. 

Our contributions can be summarized as follows:
\begin{itemize}
    \item A filtered and annotated vehicle dataset extracted from Objaverse-XL, along with embeddings, text descriptions, and vehicle sizes. 
    \item A pipeline for the automated creation of high-quality, domain-specific 3D datasets. Together with a quality-labeled dataset of rendered objects.
    \item A comprehensive evaluation demonstrating the superiority of our approach over existing filtering techniques, highlighting the importance of targeted data selection for 3D generative modeling.
\end{itemize}



